Necessary and Sufficient Budgets in Information Source Finding with Querying: Adaptivity Gap

In this paper, we study a problem of detecting the source of diffused information by querying individuals, given a sample snapshot of the information diffusion graph, where two queries are asked: {\em (i)} whether the respondent is the source or not, and {\em (ii)} if not, which neighbor spreads the information to the respondent. We consider the case when respondents may not always be truthful and some cost is taken for each query. Our goal is to quantify the necessary and sufficient budgets to achieve the detection probability $1-\delta$ for any given $0<\delta<1.$ To this end, we study two types of algorithms: adaptive and non-adaptive ones, each of which corresponds to whether we adaptively select the next respondents based on the answers of the previous respondents or not. We first provide the information theoretic lower bounds for the necessary budgets in both algorithm types. In terms of the sufficient budgets, we propose two practical estimation algorithms, each of non-adaptive and adaptive types, and for each algorithm, we quantitatively analyze the budget which ensures $1-\delta$ detection accuracy. This theoretical analysis not only quantifies the budgets needed by practical estimation algorithms achieving a given target detection accuracy in finding the diffusion source, but also enables us to quantitatively characterize the amount of extra budget required in non-adaptive type of estimation, refereed to as {\em adaptivity gap}. We validate our theoretical findings over synthetic and real-world social network topologies.

==> related.tex <==
% \subsection{Related Work}
% \label{sec:related}


\bigskip
\noindent{\bf \em Related work.}
%\smallskip
% source detection: point estimator
The research on rumor\footnote{We use the terms ``information'' and ``rumor'' interchangeably.}  source detection has recently received
significant attentions. % In this section we briefly review some related
% works that tried to solve the rumor source detection problem, in
% various settings and environments.
The first theoretical approach was done by Shah and Zaman
\cite{shah2010,shah2012,shah2010tit} and they introduced the metric
called {\em rumor centrality}, which is a simple topology-dependent
metric.  They proved that the rumor centrality describes the likelihood
function when the underlying network is a regular tree and the diffusion follows
the SI (Susceptible-Infected) model, which is
extended to a random graph network in \cite{shah2011}.  Zhu and Ying
\cite{zhu2013} solved the rumor source detection problem under the SIR
(Susceptible-Infected-Removed) model and took a sample path approach to
solve the problem, where a notion of {\em Jordan center} was introduced,
being extended to the case of sparse observations \cite{zhu2014}. Recently, there has been some
approaches for the general graphs in \cite{Kai2016, Chang2015} to find
the information source of epidemic. All the detection mechanisms so far
correspond to point estimators, whose detection performance tends to be
low.  There was several attempts to boost up the detection probability.
Wang \etal \cite{Zhang2014} showed that observing multiple different
epidemic instances can significantly increase the the detection
probability. Dong \etal \cite{dong2013} assumed that there exist a
restricted set of source candidates, where they showed the increased
detection probability based on the MAPE (maximum a posterior estimator).
Choi \etal \cite{Choi2016,Choi2016w} showed that the anti-rumor spreading under
some distance distribution of rumor and anti-rumor sources helps finding
the rumor source by using the MAPE.
The authors in \cite{bubeck2014, Khim14,Moon2016} introduced the notion of {\em
  set estimation} and provide the analytical results on the detection
performance. Choi \etal \cite{Choi17,Moon2016} first considered
the querying approach under the untruthful answer for this problem. They obtain
the sufficient number of budget to achieve the target detection probability for
the proposed MV-based algorithms. However, our work is done in a much more
generalized and practical setup in the sense that we consider the case
when users may be untruthful for both identity and direction questions, and also two types of practical querying
scenarios are studied.
There have been studies to analyze the adaptiveness gain in other literatures.
Oh \etal \cite{Sewoong16} considered the adaptiveness gain in the crowdsourcing problem
in the sense that how tasks are assigned to the workers and they showed that there is significant
adaptiveness gain compared to the non-adaptive allocation scheme. As an information maximization
problem, the authors in \cite{Singer,Yuan} considered the adaptiveness for choosing the seed nodes
after observing a partial snapshot and obtained the adaptiveness gain for maximizing the information in social network.
Our work first considers a similar adaptiveness gain on the information source detection problem
using querying under the untruthful answers.




% \begin{table}
%\renewcommand{\arraystretch}{2.4}
%\label{tab:summary}
%\center{
%    \begin{tabular}{|c||c|c|}
%    \hline
%    Query Type & Non-Adaptive & Adaptive \\ \hline \hline
%       Necessary & \large $ \frac{c(1/\delta)^{1/2}}{h(T,p,q)\log(\log (1/\delta))}$ &  \text{On-going..}\\ \cline{1-3}
%    Sufficient&     \large $ \frac{c_2 (1/\delta)}{f(\epsilon_p,\epsilon_q)\log(\log (1/\delta))}$    & \large $ \frac{c_3 (\log(1/\delta))^{\alpha}}{g (\epsilon_p,\epsilon_q)\log (\log (1/\delta))}$ \\  \hline
%  \end{tabular}
%}
%\caption{Summary of out work. (The necessary and sufficient required number of budget to guarantee that the source detection probability is at least $1- \delta$ for $0<\delta < 1$. Here, $h(T,p,q)$ is the function of entropy term for $T,p,q$ and $c_1 / \epsilon_p ^2> c_2 / f(\epsilon_p,\epsilon_q)$) where $\epsilon_p=p-1/2$ and $\epsilon_q=q-1/d$. All constants depends only on the degree $d$ and $\alpha=2$ if $p <1$ and $\alpha=1$ if $p=1$.) }
%\end{table}


% the sense
% that it belongs to a class of batch querying. Especially,
% in \cite{Khim14}, the authors
% considered the batch querying scenario which the candidate set is chosen
% by some distance $L$ from the MLE of the snapshot and obtain the
% detection probability that the source is in the chosen set.  However, to
% the best of our knowledge, our work is the first one which considers the
% untruthful feedback for both batch and interactive querying scenarios to
% detect the information source of the epidemic.


%Luo \etal \cite{Luo2013,Leng2013} considered the SI
%(Susceptible-Infected) model with limited observations, i.e., some nodes
%are infected, but not observable, where they derive an estimator
%associated with the most likely infection path that yields the observed
%subset of infected nodes with time complexity $O(n)$.

% \bigskip
% \noindent{\bf \em Organization.}
% The rest of this paper is organized as follows: In
% Section~\ref{sec:model}, we describe the system model and the
% preliminaries. Next, in Sections~\ref{sec:noninteractive} and
% \ref{sec:interactive}, we present the main results for non-interactive
% and interactive querying scenario, respectively. The proofs of main
% theorems will be described in Section~\ref{sec:proof}, followed by the
% proofs of important lemmas in Section
% \ref{sec:lemma}. Section~\ref{sec:numerical} is devoted to
% demonstrating our theoretical findings through various numerical results, and
% finally, we conclude in Section~\ref{sec:conclusion}.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

